Efficient Best-Response Computation for Strategic Network Formation under Attack

Inspired by real world examples, e.g. the Internet, researchers have introduced an abundance of strategic games to study natural phenomena in networks. Unfortunately, almost all of these games have the conceptual drawback of being computationally intractable, i.e. computing a best response strategy or checking if an equilibrium is reached is NP-hard. Thus, a main challenge in the field is to find tractable realistic network formation models. We address this challenge by investigating a very recently introduced model by Goyal et al. [WINE'16] which focuses on robust networks in the presence of a strong adversary who attacks (and kills) nodes in the network and lets this attack spread virus-like to neighboring nodes and their neighbors. Our main result is to establish that this natural model is one of the few exceptions which are both realistic and computationally tractable. In particular, we answer an open question of Goyal et al. by providing an efficient algorithm for computing a best response strategy, which implies that deciding whether the game has reached a Nash equilibrium can be done efficiently as well. Our algorithm essentially solves the problem of computing a minimal connection to a network which maximizes the reachability while hedging against severe attacks on the network infrastructure and may thus be of independent interest.

==> Abstract.tex <==
%!TEX root = paper.tex
%\vspace{-1cm}
\begin{abstract}
	\noindent Strategic network formation models the uncoordinated creation of a network by selfish agents. Inspired by real world examples, e.g. the Internet, researchers have introduced an abundance of strategic games to study natural phenomena in networks. Most of these games have the conceptual drawback of being computationally intractable. For example, computing a best response strategy or checking whether an equilibrium is reached is \NP-hard. Thus, a main challenge in the field is to find models which incorporate many interesting features and to devise efficient algorithms for solving the entailed computational tasks. 

	
    We address this challenge by providing an efficient algorithm to
    compute a best response strategy for a recently introduced model,
    thereby answering the open question posed by Goyal et
    al.~[WINE'16].  Their promising model focuses on network
    robustness by considering an adversary who attacks (and kills)
    nodes in the network and lets this attack spread virus-like to
    neighboring nodes.

    Additionally, we augment their model by introducing a less
    predictable adversary and show that our algorithm, with minor modifications, can cope with
    this more complex scenario.
	
\end{abstract}


==> Metatree.tex <==
%!TEX root = paper.tex
\subsubsection{The \metatree of $C \in \CI$}
\label{sec:mt-create}

% set of unimmunized regions
\newcommand{\URs}{\mathcal{R}_\mathcal{U}^C}
% set of immunized regions
\newcommand{\IRs}{\mathcal{R}_\mathcal{I}^C}

% single unimmunized region
\newcommand{\UR}{R_\mathcal{U}}
% single immunized region
\newcommand{\IR}{R_\mathcal{I}}
% single region is simlpy: R


To ease the strategy selection, we create an auxiliary graph to identify sets of nodes which offer equivalent benefits with respect to connection.
This graph is a bipartite tree which we call the \metatree of $C$.
Its main property states that it consists of \textbf{vulnerable} regions which stay connected when attacked and \textbf{immunized} regions which disconnect the tree when attacked.
Its construction procedure and proof of propoerties can be found at Appendix \ref{sec:mt-construction}.


\noindent In Fig.~\ref{fig:sample-metas} a conversion of a graph component through the corresponding \metagraph into the \metatree is shown. We now use the \metatree to identify the strategy maximizing the expected profit for $\ap$ when buying edges into it.
\begin{figure}[htb]
	\centering
	\includegraphics[width=4cm]{sample-graph.pdf}
	\hfill
	\includegraphics[width=4cm]{sample-metagraph.pdf}
	\hfill
	\includegraphics[width=2.7cm]{sample-metatree.pdf}

	~

	\hfill
	\includegraphics{vulnerable.pdf} {\small vulnerable}
	\hfill
	\includegraphics{targeted.pdf} {\small targeted}
	\hfill
	\includegraphics{mixed.pdf} {\small mixed}
	\hfill
	\includegraphics{immunized.pdf} {\small immunized}
	\hfill
	\caption{A graph component (left), the corresponding \metagraph (center) and the obtained \metatree (right).}
	\label{fig:sample-metas}
\end{figure}



